Agile Islands in a Waterfall Environment: Requirements Engineering Challenges and Strategies in Automotive

[Context & motivation] Driven by the need for faster time-to-market and reduced development lead-time, large-scale systems engineering companies are adopting agile methods in their organizations. This agile transformation is challenging and it is common that adoption starts bottom-up with agile software teams within the context of traditional company structures. [Question/Problem] This creates the challenge of agile teams working within a document-centric and plan-driven (or waterfall) environment. While it may be desirable to take the best of both worlds, it is not clear how that can be achieved especially with respect to managing requirements in large-scale systems. [Principal ideas/Results] This paper presents an exploratory case study at an automotive company, focusing on two departments of a large-scale systems company that is in the process of company-wide agile adoption. [Contribution] We present challenges related to requirements engineering that agile teams face while working within a larger plan-driven context and propose potential strategies to mitigate the challenges. Challenges relate to, e.g., development teams not being aware of the high-level requirement and dealing with flexibility of writing user stories. We found that strategies for overcoming most of these challenges are still lacking and thus call for more research.

==> conclusion.tex <==
% !TEX root = main.tex
\section{Conclusion}\label{concl}
We present results of the coexistence of agile methods and traditional, plan-driven methods at two departments of an automotive company.
By studying the requirements flow 
%process 
with focus on the roles and structures used to get the requirements across, we were able to identify challenges brought about by such coexistence. % of an agile and plan-driven environment.
%in that way of working. 
In both departments, and basing on the challenges observed, this coexistence of agile and plan-driven approaches seems to limit the \chg{product quality}
{efficiency of development}.
\eric{I do not see any indication that the quality suffers. Just the need to put in a lot of additional effort to get it right in the end. }
The departments have different %self-defined 
ways of working and use different tools. 
Each team implements agile methods in their own way, which leads to some differences in the challenges we observed. 
Generally, all challenges relate to working with requirements updates when the team is using agile methods while the department structure is plan-driven. 
%
% Cannot afford paragraph here.
% 
Strategies to mitigate these challenges range from having cross-functional teams, improving traceability through adequate tooling to improving process understanding and having well defined roles. 
\eric{Empower teams to manage requirements on their end?}
%All of which still fall at both ends of agile and plan-driven development. 
Practitioners in similar settings can use our results to facilitate process improvement and to drive agile transformations.
Future research will have to show to which extent these or other solutions can mitigate the challenges and to get most out of the combination of agile and plan-driven approaches.


%make better informed decisions and future work on this research can focus on addressing the challenge of requirements updates in such an environment with both agile and plan-driven teams.  

%\rashidah{The focus on the requirements engineering process should be better starting from the earliest stages of the paper. In the end, the challenges are mostly related to communication of requirements (including access to requirements, responsibilities for modifications, …) as well as requirements traceability. So I think the paper fits the scope of REFSQ but the presentation should be improved to better highlight the focus on requirements engineering.
%Also, the requirements engineering process used in the company is to me not sufficiently detailed in the paper. Better explaining what the “requirements model” is, how it is expressed/represented, and the difference practitioners make between this model and the user stories would be welcome. }
